Risk of Transfer Learning and its Applications in Finance

Transfer learning is an emerging and popular paradigm for utilizing existing knowledge from previous learning tasks to improve the performance of new ones. In this paper, we propose a novel concept of transfer risk and and analyze its properties to evaluate transferability of transfer learning. We apply transfer learning techniques and this concept of transfer risk to stock return prediction and portfolio optimization problems. Numerical results demonstrate a strong correlation between transfer risk and overall transfer learning performance, where transfer risk provides a computationally efficient way to identify appropriate source tasks in transfer learning, including cross-continent, cross-sector, and cross-frequency transfer for portfolio optimization.

==> sub-tex/feasibility.tex <==
\section{ Feasibility of Transfer Learning as an Optimization Problem}

The above optimization reformulation of the three-step transfer learning procedure provides a unified framework to analyze the impact and implications of various transfer learning techniques. In particular, it enables analyzing the feasibility of transfer learning. We show that under appropriate technical conditions, there exists an optimal procedure for transfer learning, i.e., the pair of transport mappings $(T^{X,*},T^{Y,*})$ for \eqref{eq: doub-trans}. 



\subsection{Feasibility of Transfer Learning}
 
To facilitate the feasibility analysis, the following class of loss function $\LL_T$ is introduced.

\begin{defn}[Proper loss function]
   Let $(X,Y)$ be a pair of $\XCal_T\times\YCal_T$-valued random variables with  $Law(X_T,Y_T)\in\mathcal{P}(\XCal_T\times\YCal_T)$. A loss functional $\mathcal{L}_T$ over $A_T$ is said to be {\em proper} with respect to $(X,Y)$ if there exist a corresponding function $L_T:\YCal_T\times\YCal_T\to\mathbb{R}$ bounded from below such that for any $f\in A_T$,
    \[\LL_T(f)=\E[L_T(Y,f(X))]=\E[\E[L_T(Y,f(X))|X]];\]
    moreover, the function $\tilde L_T:\YCal_T\to\mathbb{R}$, given by
    \[\tilde L_T(y)=\E[L_T(Y,Y')|Y'=y],\quad\forall y\in\YCal_T,\]
    is continuous. 
\end{defn}
Examples of proper loss functions include mean squared error and KL-divergence and more generally the Bregman divergence \cite{banerjee2005optimality} given by
\begin{equation}\label{eqn:bregman}
    D_\phi(u,v)=\phi(u)-\phi(v)-\langle u-v,\nabla\phi(v)\rangle
\end{equation}
for some strictly convex and differentiable $\phi:\YCal\to\R$,
assuming that the first and second moments of $Y$ conditioned on $Y'=y$ is continuous with respect to $y$. 
 
Without loss of generality,  we shall in this section assume the input transport set $\T^X$ contains all functions from $\XCal_T$ to $\XCal_S$. We then specify the following assumptions for the well-definedness of \eqref{eq: doub-trans}.
\begin{asp}\label{asp:A}
\begin{enumerate}
    \item $\LL_T$ is a proper loss functional with respect to $(X_T,Y_T)$;
    \item the image $f_S^*(\XCal_S)$ is compact in $(\YCal_S,\|\cdot\|_{\YCal_S})$;
    \item the set $\T^Y\subset\mathcal{C}(\XCal_T;\YCal_T)$ is such that the following set of functions
    \[\tilde\T^Y=\{\tilde T^Y:\XCal_T\to\YCal_T\,|\,\exists T^Y\in\T^Y\text{ s.t. } \tilde L_T(\tilde T^Y(x))=\inf_{y\in f_S^*(\XCal_S)}\tilde L_T(T^Y(x,y)),\ \ \forall x\in\XCal_T\}\]
    is compact in $(\{f|f:{\XCal_T}\to\YCal_T\},\|\cdot\|_{\infty})$, where for any $f:\XCal_T\to\YCal_T$, $\|f\|_{\infty}:=\sup_{x\in\XCal_T}\|f(x)\|_{\YCal_T}$.
\end{enumerate}
\end{asp}
Popular choices of loss functions, such as mean squared error from the Bregman loss family, are not only proper but also strongly convex,  therefore the compactness assumptions can be removed.  
Otherwise, compactness condition can be implemented by choosing a particular family of activation functions or imposing boundaries restrictions to weights and biases when constructing machine learning models. 

Now we are ready to establish the following feasibility result.
\begin{thm}\label{thm:existence}
    There exists an optimal solution $(T^{X,*},T^{Y,*})\in\T^X\times\T^Y$ for optimization problem \eqref{eq: doub-trans} under Assumption \ref{asp:A}.
\end{thm}
\begin{proof}[Proof of Theorem \ref{thm:existence}]
Since $\LL_T$ is proper, there exists a function $L_T:\YCal_T\times\YCal_T\to\mathbb{R}$ such that 
\[\inf_{(y,y')\in\YCal_T\times\YCal_T}L_T(y,y')>-\infty,\]
and
\[\LL_T(T^Y(\cdot,(f_S^*\circ T^X)(\cdot)))=\E[L_T(Y_T,T^Y(X_T,(f_S^*\circ T^X)(X_T)))],\quad \forall T^X\in\T^X,\,T^X\in\T^X.\]
Therefore, for the function $\tilde L_T(\cdot)=\E[L_T(Y,Y')|Y'=\cdot]$, there exists $m\in\R$ such that $\tilde L_T(y)\geq m$ for any $y\in\YCal_T$.

Now fix any $T^Y\in\T^Y$. The continuity of $\tilde L_T$ and the continuity of $T^Y(x,\cdot)$ for each $x\in\XCal_T$ guarantee the continuity of $\tilde L_T(T^y(x,\cdot))$. Together with the compactness of $f_S^*(\XCal_S)$, we have that for any $x\in\XCal_T$, 
\begin{equation}\label{eq:min-1}
M^x_{T^Y}:=\argmin_{y\in f_S^*(\XCal_S)}\tilde L_T(T^Y(x,y))\neq\emptyset.
\end{equation}
Therefore, for any $T^Y\in\T^Y$ and its corresponding $\tilde T^Y\in\tilde\T^Y$, one can construct $\tilde T^{X}\in\T^X$ such that $f_S^*(\tilde T^X(x))\in M^x_{T^Y}$ for any $x\in\XCal_T$ and hence we have
\[\min_{T^X\in\T^X}\LL_T(T^Y(\cdot,(f_S^*\circ T^X)(\cdot)))=\E[\tilde L_T(\tilde T^Y(X_T))]=:\tilde\LL_T(\tilde T^Y).\]
The continuity of the new loss functional $\tilde\LL_T$ comes from the continuity of the function $\tilde L$, and the particular choice of the function space $(\{f|f:{\XCal_T}\to\YCal_T\},\|\cdot\|_{\infty})$, where $\{f|f:{\XCal_T}\to\YCal_T\}$ contains all functions from $\XCal_T$ to $\YCal_T$. Since $\tilde\T^Y$ is compact in $(\{f|f:{\XCal_T}\to\YCal_T\},\|\cdot\|_{\infty})$, the minimum over $\tilde\T^Y$ is attained at some $\tilde T^{Y,*}$. According to the definition of $\tilde\T^Y$, there exists $T^{Y,*}\in\T^Y$ such that $\tilde\LL_T(\tilde T^{Y,*}(\cdot))=\inf_{y\in f_S^*(\XCal_S)}\tilde\LL_TT^{Y,*}(\cdot,y)$. Let $T^{X,*}$ be the $\tilde T^X\in\T^X$ corresponding to $T^{Y,*}$. For any $T^X\in\T^X$ and $T^Y\in\T^Y$, we have
\[\begin{aligned}
    \LL_T(T^Y(\cdot,(f_S^*\circ T^X)(\cdot)))&\geq \LL_T(T^Y(\cdot,(f_S^*\circ \tilde T^X)(\cdot)))\\
    &=\tilde \LL_T(\tilde T^Y(\cdot))\geq \tilde\LL_T(\tilde T^{Y,*}(\cdot))\\
    &=\LL_T(T^{Y,*}(\cdot,(f_S^*\circ T^{X,*}))(\cdot))\\
    &\geq \min_{T^X\in\mathbb{T}^X,T^Y\in\mathbb{T}^Y}\LL_T\left(T^Y(\cdot, (f_S^*\circ T^X)(\cdot))\right).
\end{aligned}\]
Therefore, the transfer learning problem \eqref{eq: doub-trans} is well-defined and it attains its minimum at $(T^{X,*},T^{Y,*})$ described above. 
\end{proof}
% Instead, a sufficiently rich family of output transport mappings is needed, 
% i.e., $\T^Y=\{f|f:\XCal_T\times\YCal_S\to\YCal_T\}$, 
% such that the target optimal model $f_T^*$ can be written as
% $f_T^*(x)=T^Y(x,f_S^*(T^X(x))),\quad\forall x\in\XCal_T.$
% However, it is often difficult to verify if the set $\T^Y$ is sufficiently rich, due to the construction of neural networks as well as the choices of optimization algorithms. The compactness conditions, on the other hand, can be implemented through choosing a particular family of activation functions or imposing boundaries restrictions to weights and biases when constructing machine learning models. 
%%%%%
\subsection{Discussion on feasibility}

We now demonstrate that the feasibility analysis  puts existing transfer learning studies on a firm mathematical footing, including domain adaptation and image classification. Additionally, it provides valuable insight for feature augmentation in particular, and expands the potential for improving model performance in general. 


\paragraph{Feasibility of domain adaption.}
Following the discussion on the domain adaption problem  in Section \ref{subsec:example_revisited},  the feasibility of the transfer learning framework \eqref{eq: doub-trans} is clearly guaranteed: this is attributed to the optimality of the pretrained model $f_S^*$ inherited from the source optimization problem and the existence of an optimal transport mapping $T^{X,*}$ from $Law(X_T)$ to $Law(X_S)$. 

Furthermore, for transfer learning problems not  satisfying the usual premise of domain adaption, 
our framework enables introducing an output transport mapping, which allows for the alignment of the output distributions between the source and target tasks.

\paragraph{Feasibility of image classification.}
Take the aforementioned classification problems in Section \ref{subsec:example_revisited} as an example. In practice, cross-entropy loss is convex with respect to the predicted probability vector, and the sigmoid activation function for the classifier layer ensures the the compactness assumption on $\T^Y$. For image data, $\XCal_S$ is typically a compact subset of an Euclidean space and therefore the image set for a continuous ResNet50 network is compact in the feature space. Hence the feasibility result holds. Our feasibility analysis provides the flexibility of incorporating an input transport mapping: it is  feasible,  and in fact beneficial for effectively utilizing the transferred feature extractor as investigated in \cite{wang2022transfer}.


\paragraph{Feasibility with feature augmentation.} 
Feature augmentation refers to the process of expanding the set of features used in a machine learning problem, which plays a significant role in improving the performance and effectiveness of models \cite{volpi2018adversarial, chen2019multi,
li2021simple}. Importantly, transfer learning combined with feature augmentation can be integrated into the mathematical framework presented in Definition \ref{def:tl}, enabling the feasibility of feature augmentation to be established accordingly. Specifically, in transfer learning with feature augmentation, we consider a source task $S$ with input and output variables $X\in\XCal$ and $Y\in\YCal$. 
The target task involves predicting the same output $Y$ from $X$ along with an additional feature denoted by $Z\in\ZCal$, with:  
\begin{equation}\label{eqn:feature_aug_tl}
\text{Source task: }\min_{f:\XCal\to\YCal}\E\left[D_\phi(Y, f(X))\right],\quad \text{Target task: } \min_{f:\XCal\times\ZCal\to\YCal}\E\left[D_\phi(Y, f(X,Z))\right].    
\end{equation}
According to the feasibility result in Theorem \ref{thm:existence}, the loss functions in \eqref{eqn:feature_aug_tl} can be selected as the Bregman loss in \eqref{eqn:bregman}.
% \begin{equation}\label{eqn:bregman}
%     D_\phi(u,v)=\phi(u)-\phi(v)-\langle u-v,\nabla\phi(v)\rangle
% \end{equation}
% for some strictly convex and differentiable $\phi:\YCal\to\R$.

Moreover, the following result shows that, under the special case of ``redundant information", transfer learning with feature augmentation can be solve explicitly by finding the appropriate input and output transport mappings.
\begin{coro}\label{lem: bregman-zero-suff}
Assume $Y$ and $Z$ are independent conditioned on $X$. The optimal input and output transport mappings $(T^X, T^Y)$ in the transfer learning optimization problem \eqref{eq: doub-trans} under the feature augmentation setting \eqref{eqn:feature_aug_tl} is given by
$$T^X(x,z)=\text{Proj}_\XCal(x,z)=x,\quad \text{and}\quad T^Y(y)=\text{id}_\YCal(y)=y.$$
\end{coro}
Moreover, we have
\begin{coro}\label{lem: bregman-monotone}
Let $(T^{X,*},T^{Y,*})$ be the optimal input and output transport mappings from solving the transfer learning optimization problem \eqref{eq: doub-trans} under the feature augmentation setting \eqref{eqn:feature_aug_tl}, i.e.,
\begin{align}
\label{eqn:feature_aug_opt}
(T^{X,*},T^{Y,*})=\argmin_{T^X\in\mathbb{T}^X,T^Y\in\mathbb{T}^Y}\E\left[D_\phi\left(Y,T^Y(X,Z,(f_S^*\circ T^X)(X,Z))\right)\right],
\end{align}
where $f^*_S=\argmin_{f:\XCal\to\YCal}\E\left[D_\phi(Y, f(X))\right]$ is the optimal pretrained model. Then,
\begin{equation}\label{eqn:feature_aug_bound}
    \E\left[D_\phi\left(Y,T^{Y,*}(X,Z,(f_S^*\circ T^{X,*})(X,Z))\right)\right] \leq \E\left[D_\phi(Y,f_S^*(X))\right].
\end{equation}
\end{coro}

\begin{proof}[Proof of Corollary \ref{lem: bregman-zero-suff} and \ref{lem: bregman-monotone}]
First recall that under the Bregman loss, the optimal source and target models in \eqref{eqn:feature_aug_tl} are given by the conditional expectations $f^*_S(X)=\E[Y|X]$ and $f^*_T(X,Z)=\E[Y|X,Z]$ (see \cite{banerjee2005optimality} for more details). Then, Corollary \ref{lem: bregman-zero-suff} follows from the fact that when $Y$ and $Z$ are independent conditioned on $X$, $\E[Y|X]=\E[Y|X,Z]$. Moreover, notice that $\text{Proj}_\XCal\in\T^X$ and $\text{id}_\YCal\in\T^Y$ and Corollary \ref{lem: bregman-monotone} follows from the optimality of $(T^{X,*},T^{Y,*})$. 
\end{proof}

Corollary \ref{lem: bregman-zero-suff} suggests that if the added feature $Z$ does not provide more relevant information compared to the original feature $X$, transfer learning can be accomplished by discarding the additional feature and directly applying the pretrained model. Moreover, Corollary \ref{lem: bregman-monotone} demonstrates that incorporating additional information in transfer learning will not have any negative impact on model performance. In other words, the inclusion of supplementary information through transfer learning can, at worst, maintain the same level of model performance, and in general, can lead to performance improvement.



==> sub-tex/office31.tex <==
\section{Transfer Risk for Image Classification with Office-31}\label{sec:image_experiment}
In this section, we will demonstrate the correlation between the performance of the transfer learning scheme \eqref{eq: doub-trans} and the transfer risk \eqref{defn: trans-bene}, through numerical experimentation using the Office-31 dataset for image classification.  

\subsection{Experiment Set-up}
Recall the neural network architecture for the experiment introduced in Section \ref{subsec:example}. For each pair of the source and the target tasks, the source model is first trained using the source data, and then the fully connected layer of the pretrained model is fine tuned using half of the target data. The performance of the model is measured by the classification accuracy using the remaining of the target data.

\paragraph{Transfer risk.} Now let us define the explicit form of transfer risk for this example. Fix a source-target pair $(S,T)$. Recall that the input transport risk $\Ef^I$ is a constant since the input transport set $\mathbb{T}^X$ is a singleton set. More specifically, we define the input transport risk as 
\begin{equation}\label{eqn:office_input}
    \Ef^I:=\mathcal{W}_1(Law(X_S), Law(X_T)),
\end{equation}
which is the Wasserstein-1 distance between the empirical distribution of (resized) source images $Law(X_S)$ and the empirical distribution of (resized) target images $Law(X_T)$. Meanwhile, for any $f_{ST}\in\mathcal{I}$ \eqref{eqn:nnclass}, we define the output transport risk as $\Ef^O(f_{ST})=\mathcal{W}_1({\mathbb{P}}_{ST}, {\mathbb{P}}_T).$
Furthermore, as discussed in Section \ref{subsec:example_revisited}, the transfer risk is given by 
\begin{equation}\label{eqn:office_risk}
    \mathcal{C}(S,T)=C(\Ef^I,\min_{f_{ST}\in\mathcal{I}}\Ef^O(f_{ST})),
\end{equation}
for some function $C:\R^2\to\R$ satisfying the regularity conditions in Definition \ref{defn: trans-bene}. Note the the optimal target distribution $\mathbb{P}_T$ in the definition of $\Ef^O(f_{ST})$ is unknown {\it a priori}. Thus, as suggested by Proposition \ref{lem: w-heur}, we approximate $\Ef^O(f_{ST})$ by $\mathcal{W}_1({\mathbb{P}}_{ST}, Law(Y_T))$. Denote the approximated output transfer risk as 
\begin{equation}\label{eqn:office_out_risk}
    \widehat{\Ef}^O=\min_{f_{ST}\in\mathcal{I}}\mathcal{W}_1({\mathbb{P}}_{ST}, Law(Y_T)).
\end{equation}
Finding $\widehat{\Ef}^O$ \eqref{eqn:office_out_risk} is an optimization problem over a neural network function class $f_{ST}\in\mathcal{I}$ \eqref{eqn:nnclass}, which is solved by gradient descent in the numerical experiment. Finally, the (approximated) transfer risk is obtained by plugging $\widehat{\Ef}^O$ into \eqref{eqn:office_risk}. 


\subsection{Numerical Result}
Three different domains in Office-31 (A, D, and W) lead to $3\times 2=6$ source-target pairs in total. The accuracy, the input transport risk $\Ef^I$ \eqref{eqn:office_input}, and the output transport risk $\widehat\Ef^O$ \eqref{eqn:office_out_risk} for each pair of source and target tasks are reported in the first three rows of Table \ref{tab:office31}. Here the input transport risk is rescaled by a constant factor to achieve the same scale as the other metrics.

In order to compute the transfer risk $\mathcal{C}$ in \eqref{eqn:office_risk} given $\Ef^I$ in \eqref{eqn:office_input} and $\widehat\Ef^O$ in \eqref{eqn:office_out_risk}, an appropriate form of function $C$ in \eqref{eqn:office_risk} need to be determined. In this experiment, we search $C$ from the class of second order polynomials, so as to maximize the (absolute value of) correlation between the transfer learning accuracy and the transfer risk. In particular, we define the risk in the following form:
\begin{equation}\label{eqn:office_risk_exact}
    \mathcal{C}(S,T)=0.31\cdot\Ef^I+0.92\cdot\left(\widehat\Ef^O\right)^2.
\end{equation}
Transfer risks for all source-target pair are reported in the last row of Table \ref{tab:office31}.

\begin{table}[H]
  \centering
    \begin{tabular}{c|cccccc}
    \toprule
    \toprule
    \textbf{Metric\textbackslash{}Task} & \textbf{A-W}   & \textbf{A-D}   & \textbf{W-A}   & \textbf{W-D}   & \textbf{D-A}   & \textbf{D-W} \\
    \midrule
    \textbf{Accuracy} & 80.9\% & 83.1\% & 66.9\% & 94.5\% & 66.6\% & 87.8\% \\
    \midrule
    \textbf{Input Risk} & 0.181 & 0.263 & 0.181 & 0.148 & 0.263 & 0.148 \\
    \midrule
    \textbf{Output Risk} & 0.428 & 0.380 & 0.545 & 0.084 & 0.543 & 0.412 \\
    \midrule
    \textbf{Transfer Risk} & 0.224 & 0.214 & 0.330 & 0.052 & 0.353 & 0.201 \\
    \bottomrule
    \bottomrule
    \end{tabular}
  \caption{Accuracy and transfer risk.}
  \label{tab:office31}
\end{table}

\paragraph{Accuracy v.s. transfer risk.} Figure \ref{fig:office31} demonstrates a significant negative correlation between the transfer learning accuracy and the transfer risk: the higher the risk, the lower the transfer learning accuracy. For example, it can be observed from Figure \ref{fig:office31} that transfer learning between DSLR and Webcam (D-W or W-D) results in low risk and high accuracy; while transfer learning from those domains to Amazon (D-A or W-A) is risky and suffers from low accuracy. Those numerical findings demonstrate the potential of transfer risk as an informative metric for the effectiveness of transfer learning task.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/acc_risk.png}
    \caption{Accuracy and transfer risk.}
    \label{fig:office31}
\end{figure}

\paragraph{Computational benefit of  transfer risk.}  

In this numerical experiment on the Office-31 dataset, assessing transfer risk is computationally efficient and guaranteed by the early-stopping trick in deep learning: for each source-target pair, the optimization problem \eqref{eqn:office_out_risk} is solved by running the gradient descent for a small and fixed number ($\sim$10) of epochs, while the transfer learning problem is solved until the accuracy converges, which may take up to  100 epochs. This early stopping trick is essentially equivalent to shrinking the search space of the output mapping from  $\mathbb{T}^Y$ in \eqref{eqn:nnclass} to some smaller class of neural networks $\mathbb{T}_0^Y\subset\mathbb{T}^Y$. 

Indeed, as emphasized in Section \ref{subsec:def_risk}, computing transfer risk \eqref{eqn:risk} is to solve an optimization problem  over the sets $\mathbb{T}^X_0$ and $\mathbb{T}^Y_0$, which can be much smaller than the function classes $\mathbb{T}^X$ and $\mathbb{T}^Y$ involved in the transfer learning problem \eqref{eq: doub-trans}. This reduction of the function classes demonstrates the potential and benefit of adopting transfer risk for  computational efficiency:  one can first perform the much easier computing task of the transfer risk, and then assess whether or not to resort to the full-scale and more computationally intense form of transfer learning.



